GradNorm: Gradient Normalization for Adaptive Loss Balancing in Deep Multitask Networks

Deep multitask networks, in which one neural network produces multiple predictive outputs, can offer better speed and performance than their single-task counterparts but are challenging to train properly. We present a gradient normalization (GradNorm) algorithm that automatically balances training in deep multitask models by dynamically tuning gradient magnitudes. We show that for various network architectures, for both regression and classification tasks, and on both synthetic and real datasets, GradNorm improves accuracy and reduces overfitting across multiple tasks when compared to single-task networks, static baselines, and other adaptive multitask loss balancing techniques. GradNorm also matches or surpasses the performance of exhaustive grid search methods, despite only involving a single asymmetry hyperparameter $\alpha$. Thus, what was once a tedious search process that incurred exponentially more compute for each task added can now be accomplished within a few training runs, irrespective of the number of tasks. Ultimately, we will demonstrate that gradient manipulation affords us great control over the training dynamics of multitask networks and may be one of the keys to unlocking the potential of multitask learning.

==> appendices.tex <==
\newpage
%https://arxiv.org/pdf/1706.05098.pdf <-- overview of multitask learning. good for literature search.
\begin{appendices}
\section{General Training Characteristics} \label{sec:training_chars}
All runs are trained at a batch size of 24 across 4 Titan X GTX 12GB GPUs and run at 30fps on a single GPU at inference. NYUv2 runs begin with a learning rate of 2e-5. Expanded NYUv2 runs last 80000 steps with a learning rate decay of 0.2 every 25000 steps. Downsampled NYUv2 runs last 20000 steps with a learning rate decay of 0.2 every 6000 steps. Updating $w_i(t)$ is performed at a learning rate of 0.025 for both GradNorm and the uncertainty weighting (\cite{kendallarxiv}) baseline. All optimizers are Adam, although we find that GradNorm is insensitive to the optimizer chosen. We implement GradNorm using TensorFlow v1.2.1. 

\section{Effects of tuning the asymmetry $\alpha$} \label{sec:alpha_tuning}
The only hyperparameter in our technique is the asymmetry $\alpha$. The optimal value of $\alpha$ for NYUv2 lies near $\alpha=1.5$, while in the highly symmetric toy example in Section \ref{sec:toy_example} we used $\alpha = 0.12$. This observation reinforces why we call $\alpha$ an asymmetry parameter. 

\begin{figure}[htb!]
	\centering
	\includegraphics[width=\textwidth]{figures/alpha_profiles.png}
	\caption{\textbf{Weights $w_i(t)$ during training, expanded NYUv2.} Traces of how the task weights $w_i(t)$ change during training for two different values of $\alpha$. A larger value of $\alpha$ pushes weights farther apart, leading to less symmetry between tasks.}
	\label{fig:tuning_alpha}
\end{figure}

Tuning $\alpha$ leads to performance gains, but we found that for NYUv2, almost any value of $0<\alpha<3$ will improve network performance over an equal weights baseline. Figure $\ref{fig:tuning_alpha}$ shows that higher values of $\alpha$ tend to push the weights $w_i(t)$ further apart, which more aggressively reduces the influence of tasks which overfit or learn too quickly (in our case, depth). Remarkably, at $\alpha=1.75$ (not shown) $w_{\text{depth}}(t)$ is suppressed to below 0.02 at no detriment to network performance on the depth task. 
\end{appendices}
\end{document}

